Optimizing Fund Allocation for Game-based Verifiable Computation Outsourcing

This paper considers the setting where a cloud server services a static set or a dynamic sequence of tasks submitted by multiple clients. Every client wishes to assure honest execution of tasks by additionally employing a trusted third party (TTP) to re-compute the tasks with a certain probability. The cloud server makes a deposit for each task it takes, each client allocates a budget (including the wage for the server and the cost for possibly hiring TTP) for each task submitted, and every party has its limited fund for either deposits or task budgets. We study how to allocate the funds optimally to achieve the three-fold goals: a rational cloud server honestly computes each task; the server's wage is maximized; the overall delay for task verification is minimized. We apply game theory to formulate the optimization problems, and develop the optimal or heuristic solutions for three application scenarios. For each of the solutions, we analyze it through either rigorous proofs or extensive simulations. To the best of our knowledge, this is the first work on optimizing fund allocation for verifiable outsourcing of computation in the setting of one server and multiple clients, based on game theory.

==> dynamicTasks.tex <==

\section{Multiple Clients with Dynamic Tasks}



To better evaluate our proposed allocation algorithms, we extend the static tasks set to dynamic flow of tasks. In the dynamic tasks setting, two algorithms are introduced for funds 
releasing.
One is the sequential releasing and the other is to release funds parallel. The details are presented as in the following sections.

\subsection{Sequential Releasing Algorithm}
In the sequential releasing scheme, tasks are assigned funds deposit one by one and only when the previous task is fully finalized, the funds will be released and the next task can be processed.
The sequential releasing algorithm is presented in Algorithm~\ref{alg:sequential} which is consisted of three parts. 

First, we initialize two buffers, buffer $B_{streamed}$ is used to store the dynamically coming tasks, buffer $B_{computed}$ is used to store the computed tasks. 

Then server runs two threads for task computation and funds allocation and releasing. 
Basically, in Thread I, each incoming task $t_{i,j}$ first stored in $B_{streamed}$ and server immediately computes it as we assume server has enough computation resources such that each incoming task can be computed parallel. 
Once the task is finished computation, it's added into $B_{computed}$ and waiting for funds allocation. 

Thread II describes the steps for funds allocation and sequentially releasing. When task is computed and saved in $B_{computed}$, server retrieves one task each time from $B_{streamed}$ and allocate its deposits $d$ to it. Then server posts the allocation strategy on blockchain and client decides whether to employ a TTP based on $p_{i,j}$. If a TTP is hired, server waits interval $p_{i,j}\hat{c}_{i,j}$ for the dispute to be resolved. Server gets its deposit and wages once the results are consistent. Finally, waiting for $T_{confirmed}$ to have the transactions fully confirmed on blockchain and the fund $d$ is released. Then the next computed task can continue the funds allocation steps.

\begin{algorithm}[htb!]
\caption{Sequential Releasing (Server $S$ v.s. Client $C_i$ with dynamically coming tasks)}
\label{alg:sequential}
{\bf Input:}
\begin{itemize}
\item
$d$: total deposit of server $S$;
\item
task set $\{t_{i,1},t_{1,2},\cdots\}$ to be dynamically streamed in,
associated costs
$\{c_{i,1},c_{i,2},\cdots\}$ and
$\{\hat{c}_{i,1},\hat{c}_{i,2},\cdots\}$ and associated budgets $\{b_{i,1},b_{i,2},\cdots\}$;
\item
$T_{confirm}$: time interval for a task from being posted to finally confirmed on blockchain;
\item
$T_{interval}$: average time interval between two incoming task.
\end{itemize}

{\bf Phase I:} Initialization.
\begin{algorithmic}[1]
\State $B_{streamed}\leftarrow \{\}$ \Comment{buffer to store streamed tasks}
\State $B_{computed}\leftarrow \{\}$ \Comment{buffer to store computed tasks}
\end{algorithmic}

{\bf Thread I:} Compute tasks parallel.
\begin{algorithmic}[1]
\For{$t_{i,j}\in\{t_{i,1},t_{i,2},\cdots\}$}
\State $B_{streamed}$.add($t_{i,j}$)
\State thread.$ComputeTask(t_{i,j})$ \Comment{compute tasks parallel}
\EndFor
\For{$t_{i,j}\in B_{streamed}$}
\If{$t_{i,j}$ is computed}
\State $B_{computed}$.add($t_{i,j}$); $B_{streamed}$.remove($t_{i,j}$)
\EndIf
\EndFor
\end{algorithmic}

{\bf Thread II:} Allocate funds and release tasks sequentially.
\begin{algorithmic}[1]
\State $w\leftarrow 0$ \Comment{wages paid to server}
\While{$B_{computed}$ is not empty}
\State $t_{i,j}\leftarrow B_{computed}$.retrieve()
\State $d_{i,j}\leftarrow d$; $d\leftarrow0$
\State $p_{i,j}\leftarrow\frac{b_{i,j}+d_{i,j}-\sqrt{(b_{i,j}+d_{i,j})2-4c_{i,j}\hat{c}_{i,j}}}{2\hat{c}_{i,j}}$
\State $flag\leftarrow true$
\State post $t_{i,j}, d_{i,j}, b_{i,j}, p_{i,j}$ on blockchain
\If{client employs TTP}
\State wait time interval $p_{i,j}\hat{c}_{i,j}$ for TTP to verify
\If{$Res_{TTP}\neq Res_{s}$} \Comment{inconsistent results}
\State $flag \leftarrow false$
\EndIf
\EndIf
\State wait for time interval $T_{confirmed}$ 
\If{$flag$}
\State $d\leftarrow d_{i,j}$; $w\leftarrow w + w_{i,j}$
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}


\subsection{Parallel Releasing Algorithm}

The parallel releasing is to allocate funds to multiple tasks each time and each task receives partial funds of $d$. When one task is finalized, the funds allocated to itself can be released and used for the next round allocation. The allocation doesn't require all funds are released and the process is promoted when partial funds are released. The parallel releasing algorithm is presented in Algorithm~\ref{alg:parallel}.

The parallel releasing algorithm has the same initialization and computation process as in sequential releasing. The phase for funds allocation and tasks releasing is different. 
As presented in Thread II, we introduce two parameters, $\alpha$ and $\beta$. $\alpha$ describes the ratio of available funds to start a new round funds allocation. $\beta$ controls the degree of parallelism, i.e. the maximal number of tasks can be processed at each time. 
When the locked deposit is no more than $\alpha d$, we can start a new round allocation. When the workload of tasks group is greater than or equal to $\beta(d-d_{locked})$, we cannot have more tasks to process parallel. When tasks are retrieved, algorithm~\ref{alg:SingleClient} is executed and each task receives an allocation of $d_{i,j}$ and $b_{i,j}$. That is, the $d_{i,j}$ is locked until task $t_{i,j}$ is finalized. 
Client then decides whether to hire a TTP for each task based on the fund allocation. If no TTP is hired or the results are consistent, the locked funds will be released after waiting $T_{confirmed}$ for the result to be finalized regardless of other tasks' actions or results.

\begin{algorithm}[htb!]
\caption{Parallel Releasing (Server $S$ v.s. Client $C_i$ with dynamically coming tasks)}
\label{alg:parallel}

{\bf Input:}
\begin{itemize}
\item
$d$: total deposit of server $S$;
\item
task set $\{t_{i,1},t_{1,2},\cdots\}$ to be dynamically streamed in,
associated costs
$\{c_{i,1},c_{i,2},\cdots\}$ and
$\{\hat{c}_{i,1},\hat{c}_{i,2},\cdots\}$ and associated budgets $\{b_{i,1},b_{i,2},\cdots\}$;
\item
$T_{confirm}$: time interval for a task from being posted to finally confirmed on blockchain;
\item
$T_{interval}$: average time interval between two incoming task;
\item
$T_{allocate}$: time interval to periodically generate allocation strategy;
\item
$\alpha$: parameter control the lower bound of released funds required for a new round funds allocation;
\item
$\beta$: parameter control the upper bound of the number of tasks to allocate funds parallel.
\end{itemize}

{\bf Phase I:} same as Algorithm~\ref{alg:sequential} Phase I

{\bf Thread I:} same as Algorithm~\ref{alg:sequential} Thread I

{\bf Thread II:} Allocate funds and release tasks parallel
\begin{algorithmic}[1]
\State $d_{locked}\leftarrow 0$ \Comment{deposits locked by system}
\State $w\leftarrow 0$ \Comment{wages paid to server}
\While{$B_{computed}$ is not empty}
\State $temp\leftarrow \{\}$ \Comment{buffer to store the retrieved tasks}
\State $\hat{c}\leftarrow 0$ \Comment{total workload of parallel tasks}
\While{every interval $T_{allocate}$ or $d_{locked}\leq\alpha*d$}
\If{$B_{computed}$ is not empty}
\State $t_{i,j}\leftarrow B_{computed}$.get()
\State $\hat{c}\leftarrow\hat{c}+\hat{c}_{i,j}$
\EndIf
\If{$\hat{c}\geq\beta(d-d_{locked})$}
\State break
\EndIf
\If{$B_{computed}$ is not empty}
\State $B_{computed}$.remove($t_{i,j}$); $temp$.add($t_{i,j}$)
\EndIf
\EndWhile
\State $d_{locked}\leftarrow d$
\State $\{b_{i,j},\cdots\}, \{d_j,\cdots\}\leftarrow$ Algorithm~\ref{alg:SingleClient} on tasks set $temp$
\For{$t_{i,j}\in temp$}
{\bf thread:}\Comment{parallel release deposits}
\State $flag_j\leftarrow true$
\If{employ TTP based on $p_{i,j}$}
\State wait for time interval $p_{i,j}\hat{c}_{i,j}$ for TTP to verify
\If{$Res_{TTP}\neq Res_{s}$} \Comment{inconsistent results}
\State $flag_j \leftarrow false$
\EndIf
\EndIf
\State wait for time interval $T_{confirmed}$
\If{$flag_j$}
\State $d_{locked}\leftarrow d_{locked}-d_{j}$ ; $w\leftarrow w+w_{i,j}$
\EndIf
\EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsection{Evaluations}


To test and evaluate sequential releasing and parallel releasing, we simulate the execution and allocation process of dynamical flow of tasks with Algorithm~\ref{alg:sequential} and~\ref{alg:parallel}. 

Detailedly, 50 group of tasks and each group with 100 tasks are introduced and simulate the dynamical flow with an average time interval $\tau=5$ which follows a Poisson distribution.
The variables in the evaluation include: 
(i) $c$ : the cost of each regular task, $c\in\{8\tau,16\tau,32\tau,64\tau,128\tau\}$, with $32\tau$ as the default value. 
(ii) $T_{confirm}$: time interval for the distribution of funds to be confirmed on blockchain, $T_{confirm}\in\{0.25\tau,0.5\tau,1\tau,2\tau,4\tau,8\tau,16\tau\}$, with $2\tau$ as the default value. 
(iii) $b$ : the budget of each task, $b\in\{2c,2.5c,3c,3.5c,4c\}$ with $2.5c$ as the default value. (vi) $p_{heavy}$ : the probability of a task to be a heavy task. $p_{heavy}\in\{0.01,0.05,0.1,0.2,0.3\}$ with a default value of $0.1$.
The heavy task has a cost $c_{heavy}$ which is $3$ times of a regular task.
The default cost of raising TTP of task with cost $c$ is $\hat{c}=3c$.
The total deposits for server is $d=\frac{c}{\tau}*120$.

We measure the following matrix: 
(i) $\frac{w}{b}$ : the ratio of wages earned by server from honest computation over total budgets provided by client, 
(ii) delay : the delay from a task being proposed until it is finalized, the delay includes four parts: the computation delay $kc$ for a task to be computed where assume $k=1$, the release delay that is the delay waiting to be allocated with deposit after computation, the TTP delay caused by raising a TTP to check the result and the confirmation delay which is the time interval to have funds distribution confirmed on blockchain. 
For each task, the computation delay and confirmation delay is fixed based on the task and system property. 
The release and TTP delay rely on the budget and deposit assigned. 
In the following evaluations, the delay represents the total delay per $\tau$ that is $delay/{\tau}$.

We first evaluate how parameters $\alpha$ and $\beta$ affect the performance of parallel releasing and then compare the results between sequential releasing and parallel releasing.
\begin{figure}[htb!]
\includegraphics[width=.474\columnwidth]{beta/beta-delay.png}
\includegraphics[width=.48\columnwidth]{beta/beta-wage.png}
\caption{delay and $\frac{w}{b}$ v.s. $\beta$}
\label{fig:alpha_and_beta}
\end{figure}
As described in Algorithm~\ref{alg:parallel}, $\alpha$ is introduced to control when to start a new round allocation based on the ratio of released funds in the system and $\beta$ is utilized to control how many tasks can be processed at the same time. 
When $\alpha=0$, that is, only when all funds are released, can a new round allocation proceed. 
$\alpha=0.3$ and $\alpha=0.6$ mean that the locked(unreleased) funds are less than $0.3d$ and $0.6d$ respectively. 
And $\alpha=1$ means no constraint on the current released deposit in the system.
Figure~\ref{fig:alpha_and_beta} shows the change of delay and $wage/budget$ with different $\alpha$ and $\beta$ when $c=32\tau$, $\tau=5$, $p_{heavy}=0.1$, , $c_{heavy}=3c$, $b=2.5c$ and $\hat{c}=3c$. 
The delay decreases as $\beta$ increase when $\alpha=0.6$ and 1.
When $\alpha=0$, the delay increases as $\beta$ increases. 
As greater $\beta$ results in the scenario: more tasks are processed parallel, since it still needs to wait for all tasks released to proceed to next allocation as $\alpha=0$, the probability of raising TTP as well as the releasing delay are increased.
When $\alpha=0.3$, as long as the released funds is no less than $0.7d$, the allocation can proceed. With the increase of $\beta$, the TTP delay increases and the releasing delay decreases. The total delay first decreases and then increases.

For ratio $\frac{w}{b}$, as expected, the greater the $\beta$ is, the smaller is the ratio. When $\beta$ increases, the degree of parallelism increases which means more tasks can be processed at the same time which in turn leads to lower deposits allocated to each task since the total funds is fixed. 
The value of $\alpha$ doesn't change the overall value of $\frac{w}{b}$ and when $\alpha=1$ the delay is smallest. Thus, we could remove the constraint of when to start a new round allocation and set $\alpha=1$ and allocate funds to task as long as there is funds released and the total workload of tasks is no more than $\beta(d-d_{locked})$.
In order to better describe the effect of $\beta$ on the parallel scheme, we present the changes of release delay and TTP delay as $\beta$ varies in Figure~\ref{fig:beta}. 
When $\beta$ increases, more tasks can be processed at the same time, the release time for tasks is decreased. 
However, the deposit assigned to each task is decreased which leads to higher probability of raising TTP and thus the TTP delay increases. In following experiments, we set $\alpha=1$ and $\beta=0.6$ for parallel releasing.
\begin{figure}[htb!]
\includegraphics[width=.48\columnwidth]{beta/beta-release-delay.png}
\includegraphics[width=.47\columnwidth]{beta/beta-ttp-delay.png}
\caption{release delay and TTP delay v.s. $\beta$}
\label{fig:beta}
\end{figure}

In Figure~\ref{fig:cost}, when $T_{confirm}=2\tau$, $p_{heavy}=0.1$, $b=2.5c$, $\hat{c}=3c$, $c\in\{8\tau,16\tau,32\tau,64\tau,128\tau\}$ and $d\in\{960,1920,3840,7680,15360\}$, delay increase with the increment of task costs. It indicates the heavier each task is, the longer it takes to finish the computation both in sequential setting and parallel setting. Compared with sequential setting, parallel has less computation delay and also smaller wage which can be explained as follows: in sequential setting, each task gets all available deposits which brings a higher wage for executor and all subsequent tasks need to wait for the current processing task to be finished which make the delay larger.
\begin{figure}[htb!]
\includegraphics[width=.48\columnwidth]{cost/cost-delay.png}
\includegraphics[width=.48\columnwidth]{cost/cost-wage.png}
\caption{delay and $\frac{w}{b}$ v.s. cost}
\label{fig:cost}
\end{figure}

\begin{figure}[htb!]
\includegraphics[width=.48\columnwidth]{confirmtime/confrimtime-delay.png}
\includegraphics[width=.48\columnwidth]{confirmtime/confrimtime-wage.png}
\caption{delay and $\frac{w}{b}$ v.s. confirm time}
\label{fig:confirmtime}
\end{figure}
Figure~\ref{fig:confirmtime} shows how the delay and wage vary as the confirm time when $c=32\tau$, $\hat{c}=3c$, $b=2.5c$, $d=3840$ and $T_{confirm}\in\{0.25\tau,0.5\tau,1\tau,2\tau,4\tau,8\tau,16\tau\}$. When the confirm time increases, the delay for both sequential and parallel increase. Compared with parallel, sequential releasing has a higher delay and increases faster. The increment of confirm time doesn't affect the TTP delay. It only increases the release delay. However, the increased confirm time adds more release delay in sequential releasing compared with parallel releasing. As all subsequent tasks need to wait for previous task to finalize in sequential while parallel releasing allows the parallelism waiting of confirm time. Therefore, the release delay in sequential releasing increases faster which leads to delay increases faster in Figure~\ref{fig:confirmtime}.
The wage is not related to confirm time, thus the $\frac{w}{b}$ for sequential and parallel are remain the same when confirm time increases. The $\frac{w}{b}$ in sequential releasing is higher as each task assigned more funds.

\begin{figure}[htb]
\includegraphics[width=.47\columnwidth]{budget/budget-delay.png}
\includegraphics[width=.48\columnwidth]{budget/budget-wage.png}
\caption{delay and $\frac{w}{b}$ v.s. budget}
\label{fig:budget}
\end{figure}

\begin{figure}[htb]
\includegraphics[width=.48\columnwidth]{heavyprob/heavyprob-delay.png}
\includegraphics[width=.48\columnwidth]{heavyprob/heavyprob-wage.png}
\caption{delay and $\frac{w}{b}$ v.s. heavy probability}
\label{fig:heavyprob}
\end{figure}

Figure~\ref{fig:budget} shows the change of delay and $\frac{w}{b}$ with budget when $T_{confirm}=2\tau$, $c=32\tau$, $d=3840$ and $b\in\{2c,2.5c,3c,3.5c,4c\}$. When budget increases, the wage received by server increases, the delay on the contrary decreases. It can be explained with equation (\ref{eq:wage}). As $\frac{\partial w}{\partial b}=\frac{b+d}{2\sqrt{(b+d)^2-4c\hat{c}}}>0$, the greater the budget, the higher is the wage. Also based on equation (\ref{eq:f(x)_first_derivative}) where $x=b+d$, the higher budget, the smaller is the delay.

Figure~\ref{fig:heavyprob} shows how the delay and wage change with the probability of a task to be heavy task when $T_{confirm}=2\tau$, $c=32\tau$, $b=2.5c$, $d=3840$ and $p_{heavy}\in\{0.01,0.05,0.1,0.2,0.3\}$. When heavy probability increases, the delay for both sequential and parallel increase which is reasonable as the computation delay, the TTP delay as well as the release delay all increase. When more heavy tasks exist, the total budget in the system also increase. For sequential releasing, the wage increase but the $\frac{w}{b}$ decreases. For parallel releasing, the wage increase as $p_{heavy}$ increases and $\frac{w}{b}$ increases as well.

Regarding to the evaluation parameters and results, we conclude that in the sequential scheme, task released and allocated one by one which can achieve higher profits for server. Server bet all funds on the current task and all subsequent tasks are blocked. While in parallel scheme, server spends deposits on multiple tasks which leads to a lower delay.


==> evaluation.tex <==
\section{Simulation and Evaluation}
\label{sec::simulation-evaluation}

To evaluate our proposed solution, we consider both the static tasks configurations and the dynamically coming task settings. 
\subsection{Static Setting}
\label{sec:static}
To simulate the interaction between executor and client, we generate tasks with same computation cost, tasks with same cost to raise TTP and tasks with same $c_{full} / c$. We compare our algorithm of allocating deposits and budgets with straw-man methods including allocating evenly and allocating proportional to task workload. We compare the greedy allocation algorithm with four different allocation methods. The uniform method is to allocate budget and deposit uniformly to all tasks. The proportional to cost method is to allocate budget and deposit proportional to cost of task. The proportional to $c_{full}$ method is to allocate budget and deposit proportional to cost of raising TTP. The proportional algorithm is to allocate budget proportional to cost and allocate deposit proportional to $c_{full}$.    

We generate tasks with same cost $c$ and different ratio of $c_{full}/c$. The total budget $B = 2.5\sum c$ and the total deposit $D=2\sum c_{full}$. Figure~\ref{static:fixed-cost} shows the delay and wage for 10 tasks with cost $c=40$ and $c_{full}/c \in \{1, \cdots, 10\}$. Since each task has same cost, the uniform allocation method is exactly the same as the proportional to cost allocation.
Figure~\ref{static:fixedcost-a} compares the total delay of 10 tasks utilizing five different allocation methods. Compares with proportional to cost, proportional to $c_{full}$, uniform and proportional allocation, greedy method achieves lowest delay. Figure~\ref{static:fixedcost-b} describes the percentage of wage received over total budgets. Also greedy receives highest wage. 

\begin{figure}[htb!]
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedcost/total_delay.png}
    \caption{total delay for 10 tasks} \label{static:fixedcost-a}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedcost/total_wage.png}
    \caption{total wage / total budget} \label{static:fixedcost-b}
  \end{subfigure}%
  \hfill   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedcost/delay_cfull.png}
    \caption{delay/$c_{full}$ vs $c_{full}$/cost} \label{static:fixedcost-c}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedcost/wage_cost.png}
    \caption{wage/cost vs $c_{full}$/cost} \label{static:fixedcost-d}
  \end{subfigure}%
\caption{10 tasks with same $c=40$, $c_{full}/c=[1,\cdots,10]$} 
\label{static:fixed-cost}
\end{figure}

Figure~\ref{static:fixed-cfull} shows the delay and wage for 10 tasks with same $c_{full}=100$ and different cost $c\in\{100,90,\cdots,10\}$. Since each task has same $c_{full}$, the uniform allocation is the same as the proportional to $c_{full}$ allocation.

\begin{figure}[htb!]
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedcfull/total_delay.png}
    \caption{total delay for 10 tasks} \label{static:fixedcfull-a}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedcfull/total_wage.png}
    \caption{total wage / total budget} \label{static:fixedcfull-b}
  \end{subfigure}%
  \hfill   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
     \includegraphics[width=\columnwidth]{static/fixedcfull/delay_cfull.png}
    \caption{delay/$c_{full}$ vs $c_{full}$/cost} \label{static:fixedcfull-c}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedcfull/wage_cost.png}
    \caption{wage/cost vs $c_{full}$/cost} \label{static:fixedcfull-d}
  \end{subfigure}%
\caption{10 tasks with same $c_{full}=100$, $c=[100,\cdots,10]$} \label{static:fixed-cfull}
\end{figure}

Figure~\ref{static:fixed-ratio} shows the delay and wage comparing 10 tasks with different cost but the same $c_{full}/c$. Since task has same $c_{full}/c$, the proportional, proportional to cost, proportional to $c_{full}$ and greedy allocation are the same.

\begin{figure}[htb!]
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedratio/total_delay.png}
    \caption{total delay for 10 tasks} \label{static:fixedratio-a}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedratio/total_wage.png}
    \caption{total wage / total budget} \label{static:fixedratio-b}
  \end{subfigure}%
  \hfill   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedratio/delay_cfull.png}
    \caption{delay/$c_{full}$ vs cost} \label{static:fixedratio-c}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{static/fixedratio/wage_cost.png}
    \caption{wage/cost vs cost} \label{static:fixedratio-d}
  \end{subfigure}%
\caption{10 tasks with same $c_{full}/c=3$, $c=[10,\cdots,100]$} \label{static:fixed-ratio}
\end{figure}

The greedy algorithm receives higher wage and lower delay compared with uniform method, proportional to cost, proportional to $c_{full}$ and proportional method.



\subsection{Dynamic Setting}
For dynamically coming tasks, we consider two allocation schemes, sequentially and parallel. Both schemes compute incoming tasks parallel. We release tasks in different ways. In sequential setting, executor spends all deposits on the current task and the deposits is released until the task is finalized. In the parallel setting, executor have multiple tasks processed parallel and continue processing when part of the deposits are released. 

\begin{algorithm}[htb!]
\caption{Allocate Sequentially}
\label{sequential}
\begin{algorithmic}[1]
\State initialize a buffer to save the streamed tasks
\For{each coming task $t_i$}
\State start computation parallel
\State add to buffer ordered by the computation time
\EndFor
\While{buffer is not empty}
\State retrieve one task from buffer
\State update allocation of deposits and budgets for retrieved task
\State task owner decides to raise TTP or not
\State wait for task result to be confirmed
\If{task is finalized}
\State redistribute budgets and released deposits
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[htb!]
\caption{Allocate Periodically and Parallel}
\label{parallel}
\begin{algorithmic}[1]
\State set time interval $T$ to periodically generate the allocation strategy
\State initialize a buffer to save the streamed tasks
\For{each coming task}
\State start computation parallel
\State add to buffer ordered by the computation time
\EndFor
\State set $temp$ to be the array store the retrieved tasks
\While{every $T$ seconds or locked deposits is no more than $\alpha*D$}
\State retrieve tasks in the buffer and saved in $temp$ so that the total workload of tasks in $temp <= \beta$*available deposits 
\EndWhile
\State allocate the deposits and budgets for retrieved tasks based on algorithm~\ref{nash_equalibrium}
\For{each task in $temp$}
\State task owner parallel decides to raise TTP or not based on the allocation
\State wait for task result to be confirmed
\State redistribute budgets and released deposits
\EndFor
\end{algorithmic}
\end{algorithm}

We assume executor has enough resources for the computation. Then each task gets computed once received. Algorithm~\ref{sequential} and ~\ref{parallel} describe the workflow of sequentially release and parallel release. The life span of each task can be described as follows.
\begin{itemize}
    \item {$received$:} task received by the executor and starts computation
    \item {$computed$:} executor finishes computation and task waits to be allocated with deposit and budget. Assume the computation time take has the same value as cost.
    \item {$release$:} task is assigned with a deposit and budget and waiting for the action of client.
    \item {$rebuttal$:} client raises a trusted execution mechanism to verify the result based on the assigned deposit and budget
    \item {$confirm$:} waiting for the computation result to be confirmed
    \item {$finalized$:} redistribute deposit and reward
\end{itemize}

In the sequential scheme, tasks are computed parallel and processed sequentially, while tasks are computed and processed parallel in parallel scheme as shown in algorithm~\ref{parallel}. Specifically, we use $\alpha$ to control when to start the allocation and $\beta$ to control how many tasks can be processed at the same time. Before the comparison of sequential scheme and parallel scheme, we first evaluate how the parameters $\alpha$ and $\beta$ influence the parallel scheme. 

Figure~\ref{delay:beta} shows the change of delay and ratio of $wage/budget$ with different $\beta$ values. As expected, the greater the $\beta$ is, the delay as well as the wage decrease. When $\beta$ increases, the degree of parallelism increases which means more tasks can be processed at the same time and results in lower delay. Also when more tasks are processed with the fixed total deposits, the deposit allocated for each task decreases which leads to a lower wage. The value of $\alpha$ doesn't change the overall value of wages and when $\alpha=1$ the delay is smallest. And $\alpha=1$ means no constraint on the current available deposit in the system. Therefore, we could only consider the effect of $\beta$ on the parallelism of tasks.  

\begin{figure}[htb!]
\includegraphics[width=.474\columnwidth]{beta/beta-delay.png}
\includegraphics[width=.48\columnwidth]{beta/beta-wage.png}
\caption{Delay and Wage VS $\beta$}
\label{delay:beta}
\end{figure}

In order to better describe the effect of $\beta$ on the parallel scheme, we evaluated with 50 groups of tasks. Each group consists of 100 tasks with a cost $c=32\tau$, $\tau=5$, $p_{heavy}=0.1$, , $c_{heavy}=3c$, $B=2.5c$ and $c_{full}=3c$. We further divide the delay into two parts, release delay is the time interval from task finishes computation to be allocated with deposit and budget. TTP delay is the time interval for a task to raise a TTP to compute the results. In simulation, we take $k=1$ which means the time delay for hiring a TTP to do computation has the same value of $c^i_{full}$. When $\beta$ increases, more tasks can be processed at the same time, the release time for tasks is decreased. However, the deposit assigned to each task is decreased which leads to higher probability of raising TTP and thus the TTP delay increases.

\begin{figure}[htb!]
\includegraphics[width=.48\columnwidth]{beta/beta-release-delay.png}
\includegraphics[width=.47\columnwidth]{beta/beta-ttp-delay.png}
\caption{Release Delay and TTP Delay VS $\beta$}
\label{50groups}
\end{figure}

To test and evaluate sequential scheme and parallel schema, we simulated 100 tasks coming periodically with an average time interval $\tau=5$ which follows a Poisson distribution. 

The variables in the evaluation includes: (i) $c$ : the cost of each task, $c$ varies from $8\tau$ to $128\tau$, with $32\tau$ as the default value. (ii) $t_{confirm}$: confirm time after the resolve of TTP to the finalize of task, $t_{confirm}$ varies from $0.25\tau$ to $16\tau$, with $2\tau$ as the default value. (iii) $B$ : the budget of each task, $B$ varies from $2c$ to $4c$ with $2.5c$ as the default value. (vi) $p_{heavy}$ : the probability of a task to be a heavy task. $p_{heavy}$ varies from $0.01$ to $0.3$ with a default value of $0.1$.
The heavy task has a cost $c_{heavy}$ which is $3$ times of a regular task.
The default cost of raising TTP of task with cost $c$ is $3c$. 

We measure the following matrix: (i) $wage/budget$ : the ratio of profits earned by executor from honest computation over total budgets provided by client, (ii) delay : the delay from a task being proposed until it is finalized. 

\begin{figure}[htb!]
\includegraphics[width=.48\columnwidth]{cost/cost-delay.png}
\includegraphics[width=.48\columnwidth]{cost/cost-wage.png}
\caption{Delay and Wage VS Cost}
\label{delay:cost}
\end{figure}

In Figure~\ref{delay:cost}, when $t_{confirm}=2\tau$, $p_{heavy}=0.1$, $B=2.5c$ and $c_{full}=3c$, the wage received by executor and delay for tasks increase with the increment of cost of tasks. It indicates the heavier each task is, the longer it takes to finishes the computation both in sequential setting and parallel setting. Compared with sequential setting, parallel has less computation delay and also smaller wage which can be explained as follows: in sequential setting, each task gets all available deposits which brings a higher wage for executor and all subsequent tasks need to wait for the current processing task to be finished which make the delay larger.

\begin{figure}[htb!]
\includegraphics[width=.48\columnwidth]{confirmtime/confrimtime-delay.png}
\includegraphics[width=.48\columnwidth]{confirmtime/confrimtime-wage.png}
\caption{Delay and Wage VS Confirm time}
\label{delay:confirmtime}
\end{figure}

Figure~\ref{delay:confirmtime} show how the delay and wage vary as the confirm time. When the confirm time increases, the delay for both sequential and parallel increase. Compared with parallel, sequential release has a higher delay. Since in sequential schema, each task starts releasing only when the previous task finalizes, when the confirm time increases, all the subsequent tasks wait for higher delay to be released and the wage received by executor remains the same when confirm time increases. 

\begin{figure}[htb]
\includegraphics[width=.47\columnwidth]{budget/budget-delay.png}
\includegraphics[width=.48\columnwidth]{budget/budget-wage.png}
\caption{Delay and Wage VS Budget}
\label{delay:budget}
\end{figure}

Figure~\ref{delay:budget} shows the change of delay and wage with budget. When budget increases, the wage received by executor also increases. The delay on the contrary decreases with the increase of budget. Figure~\ref{delay:heavyprob} shows how the delay and wage vary as the probability of a task to be heavy task. As expected, higher probability results in higher delay and higher wage.  

\begin{figure}[htb]
\includegraphics[width=.48\columnwidth]{heavyprob/heavyprob-delay.png}
\includegraphics[width=.48\columnwidth]{heavyprob/heavyprob-wage.png}
\caption{Delay and Wage VS Heavy Probability}
\label{delay:heavyprob}
\end{figure}

Regarding to the evaluation parameters and results, we conclude that in the sequential scheme, task released and allocated one by one which can achieve higher profits for executor. Executor bet all deposits on the current task and all subsequent tasks are blocked. While in parallel scheme, executor spend deposits on multiple tasks which leads to a lower delay. 

==> overview.tex <==
\section{Solution Overview}
\label{sec::solution-overview}

In our proposed solution, we analyze the game between client and executor, propose algorithms to allocate budgets and deposits to tasks. 

\subsection{The Game between Client and Executor}
In this section, we present the interaction and game between client with multiple tasks and executor. The problem is modeled as an infinite extensive game with perfect information and the utility function is derived based on the allocation algorithm. To further interpret the definition of the resource allocation game, we present the game as a tuple $G=(P, A, U)$.
\begin{itemize}
    \item $P$: players set $P$, it includes client $C$ and executor $E$.
    \item $A$: action player can take to achieve a outcome. Here  player's action is to allocate deposits, i.e., client split its budget on different tasks, executor splits its deposits on different tasks.
    \item $U$: player's utility which is determined by players' actions performed, i.e., the wage received by executor or the latency client gets for the computation of all tasks.
\end{itemize}

\begin{figure}[htb!]
\includegraphics[width=\columnwidth]{figs/tree.pdf}
\caption{The game describes the strategy played by client and executor. Client is denoted as CLT and executor is denoted as EXE. Client has infinite strategies to allocate budgets while executor has infinite strategies to allocate deposits. The leftmost branch strategy for CLT is $(b_1,b^2_{base},\cdots,b^N_{base})$ where $b_1=B-\sum b^i_{base}$ which indicates that all extra budgets are allocated to task 1 and other tasks get the base budget. The general strategy for CLT is denoted as $(b_1,\cdots,b_N)$ where $B =\sum b_i$. The rightmost strategy for CLT is to allocate all extra budgets on task $N$.
For each state of executer, the leftmost and rightmost branch also indicate the two extreme allocation cases and the middle branch is the general strategy.}
\label{tree}
\end{figure}

In the game, there are two players, $P=\{C, E\}$. Assume there are $N$ tasks existed in the game and the tasks are denoted as $t_i$ for $i=1,\cdots,N$. Let $c_i$ and $c^i_{full}$ respectively be the computation cost and cost for raising TTP for task $t_i$. The total budget of client is $B$ and $B_i$ is the budget allocated for task $t_i$ which satisfies $B=\sum^N_{i=1}B_i$.
The total deposit of executor is $D$ and $D_i$ is the deposit allocated on task $t_i$ which satisfies $D=\sum^{N}_{i=1}D_i$.
Let $W_i$ denote the reward offered to an executor for the correct computation for task $t_i$ and $p_i$ be the probability of raising a TTP to verify the computation result.
In this configuration, we assume initially executor is interested in all existed tasks and all tasks will be computed. That is executor pays a minimal deposit for all tasks.
Therefore the strategy for $C$ is $A_c=\{B_1,\cdots, B_N\}$ and the strategy for $E$ is $A_e=\{D_1,\cdots,D_N\}$. Either player has infinite number of strategies since $B_i$ and $D_i$ are real numbers for $i\in\{1,\cdots,N\}$. 

\begin{figure}[htb!]
\includegraphics[width=\columnwidth, scale=0.5]{figs/protocol.pdf}
\caption{The interaction between client and executor.}
\label{protocol}
\end{figure}

For client, it can choose an action $A_c$ to allocate its budgets, with this action, executor can decide $A_e$ to allocate the deposits to maximize utility. Then client can update its strategy based on executor's action to minimize the latency. Client and executor update iteratively and finally reaches a stable state which neither client or executor has incentive to deviate its allocation strategy. The stable state is the Nash Equilibrium of the game. 
In this game, players are rational and act to maximize utilities. That is, client chooses the allocation strategy to get lower latency and executor opts to achieve higher wage so that the goal of the game is described as the following optimization problem:
\begin{gather*}
    \text{min } L \\
    \text{s.t. max } W
\end{gather*}
Here $L$ is the total latency for all tasks get computed and $W$ is the total wage for computing all tasks. Client aims to minimize $L$ and executor aims to maximize $W$. In order to solve the optimization function, we consider from both the client's and executor's  viewpoints and have client to get optimal budget allocation given executor's strategy and have executor to get optimal deposit allocation given client's strategy. The Nash Equilibrium of the game is defined as $A^*=\{B_1,\cdots, B_N, D_1,\cdots,D_N\}$ which has $U(A^*)>U(A')$ for all $A'=\{B'_1,\cdots, B'_N, D'_1,\cdots,D'_N\}$ where $B_i\neq B'_i$ or $D_i\neq D'_i$. Furthermore, the utility function is critical is deciding the choice of player and the utility function is designed based on our outsourcing model. The outsourcing contract is presented in section~\ref{outsourcing} and the allocation algorithms is described in section~\ref{allocation}.




\subsection{Outsourcing Contract}
\label{outsourcing}
Client and executor agree on a smart contract which specifies the details of outsourcing protocol. The outsourcing contract is posted on blockchain and used by client and executor to communicate and send results as well as allocate and distribute deposits. To facilitate the outsourcing process, the outsourcing contract provides the following functions to client and executor.

{\noindent\bf{Provide Tasks:}} client calls the {\em{provide-task}} function to announce a set of tasks with the basic information including task id $t_i$, cost $c$, cost to raise TTP $c_{full}$ as well as the total budget $B$. Client also sends deposit $B$ and $\sum c_{full}$ to contract while calling {\em{provide-task}} function.

{\noindent\bf{Send Deposit:}} executor calls the {\em{send-deposit}} function to send a amount of deposit $D\geq \sum c_{full}$ to take all tasks. 

{\noindent\bf{Report Results:}} executor sends computation results of task by calling {\em{report-results}} and the results is recorded on contract.

{\noindent\bf{Allocate Budgets and Deposits:}} executor runs the allocation algorithm locally and receives an strategy to allocate budget and deposit for tasks. For task allocated with a budget and deposit, a probability of raising TTP is derived.

{\noindent\bf{Employ a Trusted Computation Mechanism:}} for task that derived with a probability to raise TTP and receives computation result from executor, client may decide to raise a TTP for recompute by calling function {\em{recompute}}. 

{\noindent\bf{Resolve Computation Result:}} client provides proof and the results computed by TTP to executor if there is a dispute on the results. Otherwise, client accepts the result provided by executor. When result is accepted, the reward is paid to executor and client pays $c_{full}$ for hiring TTP. If the result is declined, executor gets nothing and the deposit is taken by client.

{\noindent\bf{Wait for Finalization:}} once the redistribution is resolved, client and executor waits for the transactions to be confirmed and then the deposit is returned back to executor.

\begin{lemma}
\label{lem-1}
As long as $W_i\geq c_i$ and $p_i\geq\frac{c_i}{W_i+D_i}$, an economically rational executor will take the action to compute honestly and submit client a correct result rather than behave dishonestly and return an incorrect result.
\end{lemma}
\begin{proof}
(by contradiction). Suppose rational executor chooses to submit an incorrect result. If executor behaves dishonestly, it will loose the deposit with probability $p_i$ and receives reward with probability $1-p_i$, that is $-p_i*D_i+(1-p_i)*W_i$. If it behaves honestly, it would get a reward of $W_i-c_i$. It must hold that $-p_i*D_i+(1-p_i)*W_i>W_i-c_i$. Therefore, $p_i<\frac{c_i}{W_i+D_i}$ which contradicts with the condition of $p_i\geq \frac{c_i}{W_i+D_i}$. 
\end{proof}

Lemma~\ref{lem-1} states that as long as the probability of raising a trusted computation mechanism reaches a threshold which is decided by the budget, deposit and task cost, a rational executor would choose to behave honestly and client is guaranteed to receive a secure computation result. With Lemma~\ref{lem-1}, we derive the allocation algorithm in section~\ref{allocation} for client to allocate budget and executor to allocate deposit to maximize the total wages and minimize the total computation delay.

% We consider two types of clients with different objectives. One type is to use up the total fixed budget $B$ and aim to minimize the total computation delay for $N$ tasks. The other type aims to minimize the total computation delay as well as the computation cost.  
\subsection{Allocation Method}
\label{allocation}
% The game between client and executor is formalized as follows.
For task $t_i$, the budget $B_i$ includes the reward paid to executor for honest computation and the cost to raise a TTP. That is,
\begin{equation}\label{budget}
    B_i = W_i + p_i*c^i_{full}
\end{equation}
Based on Lemma~\ref{lem-1}, we take the value of $p_i=\frac{c_i}{W_i+D_i}$. 
Executor aims to maximize the wage $W_i$ under the condition $B_i = W_i + \frac{c_ic^i_{full}}{W_i+D_i}$ from equation~\ref{budget}. Then it has
\[
W_i^2+(D_i-B_i)W_i+c_ic^i_{full}-B_iD_i=0
\]
That is, $W_i$ is a function of budget $B_i$ and deposit $D_i$ allocated for task $t_i$. Once the budget $B_i$ is decided by client, the wage received by executor is a function related to the deposit $D_i$ it pays for the task. 
\begin{equation}\label{wage}
    W_i = \frac{B_i-D_i+\sqrt{(B_i+D_i)^2-4c_ic^i_{full}}}{2}
\end{equation}
Also, $W_i$ is a monotonically increasing function with a gradually decreasing ratio when the deposit $D_i$ increases which is indicated in Figure~\ref{example-a}. For each task, the greater the deposit, the greater the wage.

\begin{figure}[htb!]
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{figs/wage-deposit.png}
    \caption{wage vs deposit} \label{example-a}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{figs/delay-budget.png}
    \caption{delay vs budget} \label{example-b}
  \end{subfigure}%
\caption{An example illustrates the idea of allocation algorithms}
\label{example}
\end{figure}

Since $W_i\geq c_i$, assume $B_i=\gamma_i c_i$, then we have $\gamma_i \geq 1 + \frac{c^i_{full}}{c_i + D_i} $.
Since $D_i\geq c^i_{full}$, we further have
\begin{equation}
\label{base_budget}
    \gamma_i \geq 1 + \frac{1}{1+\frac{c_i}{c^i_{full}}} 
\end{equation}
Thus we have $B_i=\gamma_i c_i$, $\gamma_i \geq 1 + \frac{1}{1+\frac{c_i}{c^i_{full}}}$ and $D_i\geq c^i_{full}$ which indicate that the budget allocated to task $t_i$ should be at least $(1 + \frac{1}{1+\frac{c_i}{c^i_{full}}})c_i$ and the deposit allocated should be at least $c^i_{full}$ to guarantee that the computation cost can be covered by the wages received when executor is only willing to pay for the minimal deposits. In other words, the minimal deposit for task $t_i$ is $D_{base}=c^i_{full}$ and the minimal budget is $B_{base}=(1 + \frac{1}{1+\frac{c_i}{c^i_{full}}})c_i \leq 2c_i$.

Based on Equation~\ref{budget} and~\ref{wage}, then the probability $p_i$ to raise a TTP for task $t_i$ can be described as a function of budget $B_i$ and deposit $D_i$.
\begin{equation}\label{prob}
    p_i = \frac{B_i+D_i-\sqrt{(B_i+D_i)^2-4c_ic^i_{full}}}{2c^i_{full}}
\end{equation}

We model the game among client and executor mathematically with the following optimization problem. Client needs to find a strategy of allocating total budget on different tasks while the executor needs to find an optimal strategy of allocating total deposit on different tasks. Specifically, the framework models two levels of optimization. The outer level optimizes the total computation delay of all tasks while the inner level optimizes the total wages received by executor. That is,
\begin{gather*}
    \text{min } k\sum^N_{i=1} p_i c^i_{full} \\
    \text{s.t. max } \sum^N_{i=1} W_i 
\end{gather*}

Considering from executor's viewpoint, when a budget is assigned to a task by the client, it can find an optimal strategy to allocate the deposits on different tasks based on equation~\ref{wage}. To be specific, the inner level optimization can be characterized as follows.
\begin{equation}\label{max_wage}
    \begin{split}
        & max\quad \sum^N_{i=1} W_i \\
        & s.t.\quad  D = \sum^N_{i=1} D_i \\
        &\quad\quad W_i = \frac{B_i-D_i+\sqrt{(B_i+D_i)^2-4c_ic^i_{full}}}{2}
    \end{split}
\end{equation}

\begin{algorithm}[htb!]
\caption{AllocateDeposit(D, unit, N, $B_N$, $C_{full}$, $C$)}\label{split_deposit}
\begin{algorithmic}[1]
\State $W \gets 0$ \Comment{sum of wage from $N$ clients}
\State $D_N \gets C_{full}$ \Comment{list, deposit for each client initial value is $C_{full}$} 
\Procedure{SplitDeposit}{D, unit, N, $B_N$, $C_{full}$}
\State $Q \gets [\, ]$ \Comment{priority queue, each item is a tuple (index, reward) and sort by reward descendent}
\State $deposit \gets D - \text{sum}(D_N) $ \Comment{deposit left to be split}
\For{client $i \in \{1,\cdots,N\}$}
\State $W \gets W + \text{getWage}(0, i)$ 
\If{$deposit>=unit$}
\State $reward \gets \text{getWage}(unit, i) - \text{getWage}(0, i)$
\State $Q.\text{Put}((i, reward)) $ 
\EndIf
\EndFor
\While{$deposit>=unit$}
\State $deposit \gets deposit - unit$
\State $elem \gets \text{Q.Get()}$
\State $idx \gets elem.\text{index}$
\State $D_N[idx] \gets D_N[idx] + unit$
\State $reward \gets \text{getWage}(unit, idx) - \text{getWage}(0, idx)$
\State $Q.\text{Put}((idx, reward))$
\State $W \gets W + elem.\text{reward}$
\EndWhile
\State \textbf{return} $W, D_N$
\EndProcedure
% extra arguments: $B_N$, $D_N$, C, $C_{full}$
\Procedure {getWage}{unit, i}
% \State $reward \gets   \frac{B_N[i]-(D_N[i]+unit)+\sqrt{((B_N[i]+D_N[i]+unit)^2-4*C[i]*C_{full}[i])}}{2*C_{full}[i]}$
\State $reward \gets W(B_N[i], D_N[i]+unit)$ \Comment{$W$ is the wage calculated based on Equation~\ref{wage}}
\State \textbf{return} $reward$
\EndProcedure
\end{algorithmic}
\end{algorithm}

Based on the characteristic of function $W_i(B_i, D_i)=\frac{B_i-D_i+\sqrt{(B_i+D_i)^2-4c_ic^i_{full}}}{2}$. We can use greedy algorithm to find out the strategy of allocating deposits for executor as well as the strategy of allocating budgets for client. 
Algorithm~\ref{split_deposit} describes the approach used by executor to find an optimal strategy to split the deposit. For each budget combination a client assigns on different tasks, executor can find an optimal strategy of deposits allocation on tasks based on algorithm~\ref{split_deposit}. In algorithm~\ref{split_deposit}, executor initially allocates a minimal deposit to all tasks and for the remaining deposits, it always choose the task which brings higher wage to assign each deposit unit. In Figure~\ref{example-a}, it gives an example illustrating how algorithm~\ref{split_deposit} works. We consider 4 tasks with different cost $c\in\{1,2,3,4\}$ and same $c_{full}=4$. The total deposits to allocate has value $2.5\sum {c_{full}}$ and each task has base budget which is derived based on equation~\ref{base_budget}. The tangent line shows the final state where each task is assigned with the deposit corresponding to the x value. In each step, the task with the highest slope at the next point is chosen to allocate the deposit unit.


\begin{algorithm}[htb!]
\caption{AllocateBudget(B, unit, N, $D_N$, $C_{full}$, $C$)}
\label{split_budget}
\begin{algorithmic}[1]
\State $Delay \gets 0$ \Comment{sum of delay for executing $N$ tasks}
\State $B_N \gets B_{base}$ \Comment{list, budget for each task initial value is calculated based on equation~\ref{base_budget}} 
\Procedure{SplitBudget}{B, unit, N, $D_N$, $C_{full}$}
\State $Q \gets [\, ]$ \Comment{priority queue, each item is a tuple (index, delay) and sort by delay ascendant}
\State $budget \gets B - \text{sum}(B_N) $ \Comment{budget left to be split}
\For{client $i \in \{1,\cdots,N\}$}
\State $Delay \gets Delay + \text{getDelay}(0, i)$ 
\If{$budget>=unit$}
\State $delay \gets \text{getDelay}(unit, i) - \text{getDelay}(0, i)$
\State $Q.\text{Put}((i, delay)) $ 
\EndIf
\EndFor
\While{$budget>=unit$}
\State $budget \gets budget - unit$
\State $elem \gets \text{Q.Poll()}$
\State $idx \gets elem.\text{index}$
\State $B_N[idx] \gets B_N[idx] + unit$
\State $delay \gets \text{getDelay}(unit, idx) - \text{getDelay}(0, idx)$
\State $Q.\text{Put}((idx, delay))$
\State $Delay \gets Delay + elem.\text{delay}$
\EndWhile
\State \textbf{return} $Delay, B_N$
\EndProcedure
\Procedure {getDelay}{unit, i}
% \State $delay \gets   \frac{B_N[i]+unit+D_N[i]-\sqrt{((B_N[i]+unit+D_N[i])^2-4*C[i]*C_{full}[i])}}{2*C_{full}[i]}$
\State $delay \gets k*p(B_N[i]+unit, D_N[i])*C_{full}[i]$ \Comment{$p$ is the probability to raise TTP calculated based on equation~\ref{prob}}
\State \textbf{return} $delay$
\EndProcedure
\end{algorithmic}
\end{algorithm}

From client's point of view, the outer level optimization is further described as follows. Algorithm~\ref{split_budget} shows the approach for client to allocate the total budget.
In Figure~\ref{example-b}, 4 tasks are considered to illustrate how the delay varies when the budget changes. Tasks have same cost and different $c_{full}\in\{1,2,3,4\}$. We consider the minimal deposit assigned to each task that is $D_i=c^i_{full}$ and total budget $B=3\sum c$ and $k=1$. The tangent line shows the decreasing ratio of the final state. In each step, we choose the task which brings highest delay decreasing to assign the budget. The point showed on each line is the final budget assigned to each task. 
\begin{equation}\label{min_delay}
    \begin{split}
        & min\quad k\sum_{i=1}^N p_i c^i_{full} \\
        & s.t.\quad  p_i c^i_{full} = \frac{B_i+D_i-\sqrt{(B_i+D_i)^2-4c_ic^i_{full}}}{2} \\
        &\quad\quad B_i \geq (1 + \frac{1}{1+\frac{c_i}{c^i_{full}}})c_i \\
        & \quad\quad B = \sum^N_{i=1} B_i
    \end{split}
\end{equation}

Therefore, in this fixed budget configuration, client and executor can use greedy algorithms to find an optimal strategy to split the budget to get a minimal delay and to split deposits and get a maximal wages respectively.   

The game between server and client to find a nash equilibrium is described in algorithm~\ref{nash_equalibrium}. Initially, each task $t_i$ is randomly assigned a budget which satisfies equation $B_i= B^i_{base}$ and $B=\sum^N_{i=1}B_i$. Then server can get a optimal allocation strategy of assigning deposits on each task based on algorithm~\ref{split_deposit}. Based on the optimal strategy of allocating deposit, client update the strategy to allocate budgets based on algorithm~\ref{split_budget}.


\begin{algorithm}[htb!]
\caption{Find Nash Equilibrium}
% (B, N, $C_{full}$, $C$, $unit_b$, D, $unit_d$)
\label{nash_equalibrium}
\begin{algorithmic}[1]
% \State initialize $ B_N=[\gamma_1c_1, \gamma_2c_2, \cdots, \gamma_Nc_N]$
\State $\_, B_N \gets$ AllocateBudget(B, $unit_b$, N, $D_N$, $C_{full}$, $C$)
\State $\_, D_N \gets$ AllocateDeposit(D, $unit_d$, N, $B_N$, $C_{full}$, $C$)
\State \textbf{return} $B_N, D_N$
\end{algorithmic}
\end{algorithm}


\subsection{Analysis}

Based on equation~\ref{wage}, the wage $W_i$ executor receives for computing task $t_i$ relates to deposit $D_i$. 
Considering the characteristic of function $W_i(D_i)$, we have 
\begin{equation}\label{W-D-first}
    \diffp{W_i}{{D_i}} = \frac{1}{2}*(\frac{B_i+D_i}{\sqrt{(B_i+D_i)^2-4c_ic^i_{full}}}-1) > 0
\end{equation}
Since $B_i>W_i\geq c_i$ and $D_i\geq c_{full}^i$, then $(B_i+D_i)^2-4c_ic^i_{full}>(c_i+c^i_{full})^2-4c_ic^i_{full}=(c_i-c_{full}^i)^2\geq 0$. Thus, $W_i$ is a monotonically increasing function with respect to $D_i$. Also the second derivation of the function satisfies 
\begin{equation}\label{W-D-second}
    \pd[2]{W_i}{{D_i}} = \frac{-2c_ic^i_{full}}{(\sqrt{(B_i+D_i)^2-4c_ic_{full}^i})^3} < 0
\end{equation}
Therefore, the greedy algorithm lead to the global optimal results. The detailed proof of correctness is described in Lemma~\ref{deposit_optimal_proof}. 


\begin{equation}\label{p-B-first}
    \diffp{p_i}{{B_i}} = \frac{1}{2c^i_{full}}*(1-\frac{B_i+D_i}{\sqrt{(B_i+D_i)^2-4c_ic^i_{full}}}) < 0
\end{equation}
Since $B_i>W_i\geq c_i$ and $D_i\geq c_{full}^i$, then $(B_i+D_i)^2-4c_ic^i_{full}>(c_i+c^i_{full})^2-4c_ic^i_{full}=(c_i-c_{full}^i)^2\geq 0$. Thus, $p_i$ is a monotonically decreasing function with respect to $B_i$. Also the second derivation of the function satisfies 
\begin{equation}\label{p-B-second}
    \pd[2]{p_i}{{B_i}} = \frac{2c_i}{(\sqrt{(B_i+D_i)^2-4c_ic_{full}^i})^3} > 0
\end{equation}
Therefore, the greedy algorithm lead to the global optimal results. Refer to Lemma~\ref{budget_optimal_proof} for the correctness proof.


\begin{lemma}
\label{deposit_optimal_proof}
Given $N$ tasks from client and each task $i$ with corresponding computation cost $c_i$, cost to raise TTP $C^i_{full}$ and budget $B_i$, and a total deposit $D$ from executor, 
the strategy $S=[d_1,d_2,\cdots,d_N]$ of allocating deposits to $N$ tasks derived from algorithm~\ref{split_deposit} leads to an optimal result that achieves maximal total wages where $d_i$ is the deposit allocates to task $i$ and $D=\sum^N_{i=1}d_i$.
\end{lemma}
\begin{proof}
(Proof by contradiction.) Assume the optimal strategy is $O=[d'_1,d'_2,\cdots,d'_N]$ and $S\neq O$. Then there must exists two tasks $i, j\in \{1,2,\cdots,N\}$ that $d_i\neq d'_i$ and $d_j\neq d'_j$. WLOG, we assume $d_i>d'_i$. Rewrite the strategy $S$ in the order of adding one deposit unit to one task as indicated in the algorithm, that is $Ord(S)=[s_1,s_2,\cdots,s_i,\cdots,s_{D'}]$ where $s_i\in\{1,2,\cdots,N\}$ and $D'=D-\sum^{N}_{j=1}c_{full}^j$. And $Ord(O)=[o_1,o_2,\cdots,o_i,\cdots,o_{D'}]$ where the elements in $Ord(O)$ is ordered by the increasing wage descent. 
It also satisfies $d_i = \sum^{D'}_{j=1}\mathds{1}_{s_j=i}$ and $d'_i = \sum^{D'}_{j=1}\mathds{1}_{o_j=i}$ for $i\in\{1,2,\cdots,N\}$. 
Let $\Delta^i_s=W_{s_i}-W_{s_{i-1}}$ and $\Delta^i_o=W_{o_i}-W_{o_{i-1}}$ define the increased wage from step $i-1$ to $i$ in strategy $Ord(S)$ and $Ord(O)$ respectively. 
Then it satisfies $\Delta^1_s>\cdots>\Delta^i_s>\cdots>\Delta^{D'}_s>0$ and $\Delta^1_o>\cdots>\Delta^i_o>\cdots>\Delta^{D'}_o>0$ based on equation~\ref{W-D-first} and ~\ref{W-D-second}.
Assume index $i$ is the smallest index where $s_i\neq o_i$, it must have $o_j\neq s_i$ since the choice of $o_j$ in $Ord(O)$ is ordered by the increasing wage descendent. We can construct a strategy $O^*$ which changes $o_i$ in $O$ to $s_i$ in $S$ and the rest are the same as in $Ord(O)$. That is $Ord(O^*)=[o'_1,o'_2,\cdots,s_i,o'_{i+1},\cdots,o'_{D'}]$ which satisfies $o'_j=o_j=s_j$ for $j\in \{1,\cdots,i-1\}$ and $o'_j=o_j$ for $j\in \{i+1,\cdots,D'\}$. Then $\Delta^j_{o'}=\Delta^j_o$ for $j\in\{1,\cdots,i-1\}$.
Since strategy $S$ always choose the action which derives maximal wage in each step, then we have $\Delta^i_s>\Delta^i_o$. For $o'_j=o_i$ when $j\in \{i+1,\cdots,D'\}$, we have $\Delta^j_{o'}>\Delta^j_o$ based on equation~\ref{W-D-second}. For $o'_j\neq o_i$ when $j\in \{i+1,\cdots,D'\}$, we have $\Delta^j_{o'}= \Delta^j_o$ based on equation~\ref{W-D-second}. Then the total wage get from strategy $O^*$ is $W(O^*)=\sum^{D'}_{i=1}\Delta^j_{o'}$. The wage from $O$ is $W(O)=\sum^{D'}_{i=1}\Delta^j_o$. Based on the conditions mentioned above, we have $W(O^*)>W(O)$ which contradicts the statement that strategy $O$ is optimal. Thus, strategy $S$ outputs the optimal results.    

\end{proof}


\begin{lemma}
\label{budget_optimal_proof}
Given $N$ tasks and a total budget $B$ from client and each task $i$ with corresponding computation cost $c_i$, cost to raise TTP $C^i_{full}$, and a deposit allocation stategy $D=[d_1,\cdots,d_N]$ from executor, 
the strategy $S=[b_1,b_2,\cdots,b_N]$ of allocating budgets to $N$ tasks derived from algorithm~\ref{split_budget} leads to an optimal result that achieves minimal total delays where $b_i$ is the budget allocates to task $i$ and $B=\sum^N_{i=1}b_i$. 
\end{lemma}

\begin{proof}
(Proof by contradiction.) Assume the optimal strategy is $O=[b'_1,b'_2,\cdots,b'_N]$ and $S\neq O$. Then there must exists two tasks $i, j\in \{1,2,\cdots,N\}$ that $b_i\neq b'_i$ and $b_j\neq b'_j$. WLOG, we assume $b_i>b'_i$. Rewrite the strategy $S$ in the order of adding one budget unit to one task as indicated in the algorithm, that is $Ord(S)=[s_1,s_2,\cdots,s_i,\cdots,s_{B'}]$ where $s_i\in\{1,2,\cdots,N\}$ and $B'=B-\sum^{N}_{j=1}B^j_{base}$ where $B^j_{base}=\gamma_j c_j$. And $Ord(O)=[o_1,o_2,\cdots,o_i,\cdots,o_{B'}]$ where the elements in $Ord(O)$ is ordered by the increased delay ascendant. 
It also satisfies $b_i = \sum^{B'}_{j=1}\mathds{1}_{s_j=i}$ and $b'_i = \sum^{B'}_{j=1}\mathds{1}_{o_j=i}$ for $i\in\{1,2,\cdots,N\}$. 
Let $\Delta^i_s=p_{s_i}-p_{s_{i-1}}$ and $\Delta^i_o=p_{o_i}-p_{o_{i-1}}$ define the increased delay from step $i-1$ to $i$ in strategy $Ord(S)$ and $Ord(O)$ respectively. 
Then it satisfies $\Delta^1_s<\cdots<\Delta^i_s<\cdots<\Delta^{B'}_s<0$ and $\Delta^1_o<\cdots<\Delta^i_o<\cdots<\Delta^{B'}_o<0$ based on equation~\ref{p-B-first} and ~\ref{p-B-second}.
Assume index $i$ is the smallest index where $s_i\neq o_i$ and for $j\in\{i+1,\cdots,B'\}$, it must have $o_j\neq s_i$ since the choice of $o_j$ in $Ord(O)$ is ordered by the increasing delay ascendant. 
We can construct a strategy $O^*$ which changes $o_i$ in $O$ to $s_i$ in $S$ and the rest are the same as in $Ord(O)$. That is $Ord(O^*)=[o'_1,o'_2,\cdots,s_i,o'_{i+1},\cdots,o'_{B'}]$ which satisfies $o'_j=o_j=s_j$ for $j\in \{1,\cdots,i-1\}$ and $o'_j=o_j$ for $j\in \{i+1,\cdots,B'\}$. Then $\Delta^j_{o'}=\Delta^j_o$ for $j\in\{1,\cdots,i-1\}$.
Since strategy $S$ always choose the action which derives minimal delay in each step, then we have $\Delta^i_s<\Delta^i_o$. For $o'_j=o_i$ when $j\in \{i+1,\cdots,B'\}$, we have $\Delta^j_{o'}<\Delta^j_o$ based on equation~\ref{p-B-second}. For $o'_j\neq o_i$ when $j\in \{i+1,\cdots,B'\}$, we have $\Delta^j_{o'}= \Delta^j_o$ based on equation~\ref{p-B-second}. Then the total wage get from strategy $O^*$ is $p(O^*)=\sum^{B'}_{i=1}\Delta^j_{o'}$. The delay from $O$ is $p(O)=\sum^{B'}_{i=1}\Delta^j_o$. Based on the conditions mentioned above, we have $p(O^*)<p(O)$ which contradicts the statement that strategy $O$ is optimal. Thus, strategy $S$ outputs the optimal results.    
\end{proof}



